Safe Adaptive Feedback Control via Barrier States

This paper presents a safe feedback control framework for nonlinear control-affine systems with parametric uncertainty by leveraging adaptive dynamic programming (ADP) with barrier-state augmentation. The developed ADP-based controller enforces control invariance by optimizing a value function that explicitly penalizes the barrier state, thereby embedding safety directly into the Bellman structure. The near-optimal control policy computed using model-based reinforcement learning is combined with a concurrent learning estimator to identify the unknown parameters and guarantee uniform convergence without requiring persistency of excitation. Using a barrier-state Lyapunov function, we establish boundedness of the barrier dynamics and prove closed-loop stability and safety. Numerical simulations on an optimal obstacle-avoidance problem validate the effectiveness of the developed approach.

==> Figures/W_a.tex <==
\begin{tikzpicture}
  \begin{axis}[
    width=\linewidth,
    height=0.45\linewidth,
    xlabel={$t$ (in sec)},
    ylabel={$\hat{W_a}$},
    grid=both,
    legend style={nodes={scale=0.7, transform shape}},
    xmin = 0,
    enlarge y limits=0.01,
    enlarge x limits=0,
  ]

  % =======================================
  % Colors for each weight component
  % W_a1 = red, W_a2 = blue, W_a3 = purple,
  % W_a4 = green, W_a5 = orange, W_a6 = cyan
  % =======================================

  % ===========================
  % ======== CASE 01 ==========
  % ===========================
  \addplot+[thick, red!70!black,
      solid,
      mark=+,
      mark size=2pt,
      mark repeat=60,
      mark options={solid}]
    table[x index=0, y index=1, col sep=space]
      {Data/Case-01/Wa_hat.dat};

  \addplot+[thick, blue,
      solid,
      mark=*,
      mark size=1pt,
      mark repeat=60,
      mark options={solid}]
    table[x index=0, y index=2, col sep=space]
      {Data/Case-01/Wa_hat.dat};

  \addplot+[thick, purple!80!black,
      solid,
      mark=diamond,
      mark size=2pt,
      mark repeat=60,
      mark options={solid}]
    table[x index=0, y index=3, col sep=space]
      {Data/Case-01/Wa_hat.dat};

  \addplot+[thick, green!60!black,
      solid,
      mark=pentagon,
      mark size=2pt,
      mark repeat=60,
      mark options={solid}]
    table[x index=0, y index=4, col sep=space]
      {Data/Case-01/Wa_hat.dat};

  \addplot+[thick, orange!80!black,
      solid,
      mark=square,
      mark size=1pt,
      mark repeat=60,
      mark options={solid}]
    table[x index=0, y index=5, col sep=space]
      {Data/Case-01/Wa_hat.dat};

  \addplot+[thick, cyan!60!black,
      solid,
      mark= triangle,
      mark size=1pt,
      mark repeat=60,
      mark options={solid}]
    table[x index=0, y index=6, col sep=space]
      {Data/Case-01/Wa_hat.dat};




  % % ===========================
  % % ======== CASE 02 ==========
  % % ===========================
  % \addplot+[thick, red!70!black,
  %     dashed,
  %     mark=square*,
  %     mark size=1pt,
  %     mark repeat=60,
  %     mark options={solid}]
  %   table[x index=0, y index=1, col sep=space]
  %     {Data/Case-02/Wa_hat.dat};

  % \addplot+[thick, blue,
  %     dashed,
  %     mark=square*,
  %     mark size=1pt,
  %     mark repeat=60,
  %     mark options={solid}]
  %   table[x index=0, y index=2, col sep=space]
  %     {Data/Case-02/Wa_hat.dat};

  % \addplot+[thick, purple!80!black,
  %     dashed,
  %     mark=square*,
  %     mark size=1pt,
  %     mark repeat=60,
  %     mark options={solid}]
  %   table[x index=0, y index=3, col sep=space]
  %     {Data/Case-02/Wa_hat.dat};

  % \addplot+[thick, green!60!black,
  %     dashed,
  %     mark=square*,
  %     mark size=1pt,
  %     mark repeat=60,
  %     mark options={solid}]
  %   table[x index=0, y index=4, col sep=space]
  %     {Data/Case-02/Wa_hat.dat};

  % \addplot+[thick, orange!80!black,
  %     dashed,
  %     mark=square*,
  %     mark size=1pt,
  %     mark repeat=60,
  %     mark options={solid}]
  %   table[x index=0, y index=5, col sep=space]
  %     {Data/Case-02/Wa_hat.dat};

  % \addplot+[thick, cyan!60!black,
  %     dashed,
  %     mark=square*,
  %     mark size=1pt,
  %     mark repeat=60,
  %     mark options={solid}]
  %   table[x index=0, y index=6, col sep=space]
  %     {Data/Case-02/Wa_hat.dat};

  % % Legend entry for Case 02
  % \addlegendimage{only marks, mark=square*, mark options={solid, color=black}}
  % \addlegendentry{\small Case 02}



  % % ===========================
  % % ======== CASE 03 ==========
  % % ===========================
  % \addplot+[thick, red!70!black,
  %     dashed,
  %     mark=triangle*,
  %     mark size=1pt,
  %     mark repeat=60,
  %     mark options={solid}]
  %   table[x index=0, y index=1, col sep=space]
  %     {Data/Case-03/Wa_hat.dat};

  % \addplot+[thick, blue,
  %     dashed,
  %     mark=triangle*,
  %     mark size=1pt,
  %     mark repeat=60,
  %     mark options={solid}]
  %   table[x index=0, y index=2, col sep=space]
  %     {Data/Case-03/Wa_hat.dat};

  % \addplot+[thick, purple!80!black,
  %     dashed,
  %     mark=triangle*,
  %     mark size=1pt,
  %     mark repeat=60,
  %     mark options={solid}]
  %   table[x index=0, y index=3, col sep=space]
  %     {Data/Case-03/Wa_hat.dat};

  % \addplot+[thick, green!60!black,
  %     dashed,
  %     mark=triangle*,
  %     mark size=1pt,
  %     mark repeat=60,
  %     mark options={solid}]
  %   table[x index=0, y index=4, col sep=space]
  %     {Data/Case-03/Wa_hat.dat};

  % \addplot+[thick, orange!80!black,
  %     dashed,
  %     mark=triangle*,
  %     mark size=1pt,
  %     mark repeat=60,
  %     mark options={solid}]
  %   table[x index=0, y index=5, col sep=space]
  %     {Data/Case-03/Wa_hat.dat};

  % \addplot+[thick, cyan!60!black,
  %     dashed,
  %     mark=triangle*,
  %     mark size=1pt,
  %     mark repeat=60,
  %     mark options={solid}]
  %   table[x index=0, y index=6, col sep=space]
  %     {Data/Case-03/Wa_hat.dat};

  % % Legend entry for Case 03
  % \addlegendimage{only marks, mark=triangle*, mark options={solid, color=black}}
  % \addlegendentry{\small Case 03}



  % =======================================
  % Legend entries for each weight (colors)
  % =======================================
  \addlegendimage{thick, red!70!black}
  \addlegendentry{$\hat W_{a,1}$}

  \addlegendimage{thick, blue}
  \addlegendentry{$\hat W_{a,2}$}

  \addlegendimage{thick, purple!80!black}
  \addlegendentry{$\hat W_{a,3}$}

  \addlegendimage{thick, green!60!black}
  \addlegendentry{$\hat W_{a,4}$}

  \addlegendimage{thick, orange!80!black}
  \addlegendentry{$\hat W_{a,5}$}

  \addlegendimage{thick, cyan!60!black}
  \addlegendentry{$\hat W_{a,6}$}

  \end{axis}
\end{tikzpicture}


==> Figures/wchat.tex <==
\begin{tikzpicture}
  \begin{axis}[
    width=\linewidth,
    height=0.45\linewidth,
    xlabel={$t$ (in sec)},
    ylabel={$\hat{W_c}$},
    grid=both,
    legend style={nodes={scale=0.7, transform shape}},
    xmin = 0,
    enlarge y limits=0.01,
    enlarge x limits=0,
  ]

  % ===================================================
  % COLORS FOR COMPONENTS (same for all cases)
  % Wc1=red, Wc2=blue, Wc3=purple, Wc4=green,
  % Wc5=orange, Wc6=cyan
  % ===================================================

  % ================================
  % ========== CASE 01 =============
  % ================================
  \addplot+[thick, red!70!black,
      solid,
      mark=+,
      mark size=2pt,
      mark repeat=60,
      mark options={solid}]
    table[x index=0, y index=1, col sep=space]
      {Data/Case-01/Wc_hat.dat};

  \addplot+[thick, blue,
      solid,
      mark=*,
      mark size=1pt,
      mark repeat=60,
      mark options={solid}]
    table[x index=0, y index=2, col sep=space]
      {Data/Case-01/Wc_hat.dat};

  \addplot+[thick, purple!80!black,
      solid,
      mark=diamond,
      mark size=2pt,
      mark repeat=60,
      mark options={solid}]
    table[x index=0, y index=3, col sep=space]
      {Data/Case-01/Wc_hat.dat};

  \addplot+[thick, green!60!black,
      solid,
      mark=pentagon,
      mark size=2pt,
      mark repeat=60,
      mark options={solid}]
    table[x index=0, y index=4, col sep=space]
      {Data/Case-01/Wc_hat.dat};

  \addplot+[thick, orange!80!black,
      solid,
      mark=square,
      mark size=1pt,
      mark repeat=60,
      mark options={solid}]
    table[x index=0, y index=5, col sep=space]
      {Data/Case-01/Wc_hat.dat};

  \addplot+[thick, cyan!60!black,
      solid,
      mark= triangle,
      mark size=1pt,
      mark repeat=60,
      mark options={solid}]
    table[x index=0, y index=6, col sep=space]
      {Data/Case-01/Wc_hat.dat};


  % ==================================
  % Legend for colored lines (6 weights)
  % ==================================
  \addlegendimage{thick, red!70!black}
  \addlegendentry{$\hat W_{c,1}$}

  \addlegendimage{thick, blue}
  \addlegendentry{$\hat W_{c,2}$}

  \addlegendimage{thick, purple!80!black}
  \addlegendentry{$\hat W_{c,3}$}

  \addlegendimage{thick, green!60!black}
  \addlegendentry{$\hat W_{c,4}$}

  \addlegendimage{thick, orange!90!black}
  \addlegendentry{$\hat W_{c,5}$}

  \addlegendimage{thick, cyan!60!black}
  \addlegendentry{$\hat W_{c,6}$}

  \end{axis}
\end{tikzpicture}

